Distance Sensitive Bloom Filters Without False Negatives

A Bloom filter is a widely used data-structure for representing a set $S$ and answering queries of the form "Is $x$ in $S$?". By allowing some false positive answers (saying "yes" when the answer is in fact `no') Bloom filters use space significantly below what is required for storing $S$. In the distance sensitive setting we work with a set $S$ of (Hamming) vectors and seek a data structure that offers a similar trade-off, but answers queries of the form "Is $x$ close to an element of $S$?" (in Hamming distance). Previous work on distance sensitive Bloom filters have accepted false positive and false negative answers. Absence of false negatives is of critical importance in many applications of Bloom filters, so it is natural to ask if this can be also achieved in the distance sensitive setting. Our main contributions are upper and lower bounds (that are tight in several cases) for space usage in the distance sensitive setting where false negatives are not allowed.

==> avg_upper.tex <==
\subsection{Average error}
\begin{theorem}
\label{thm:upperbound}

A $(r>0,c>0,\epsilon>0)$-distance-sensitive approximate membership filter with guarantees on the average error requires space:

\begin{align}
\BO{n\Big(\log\big(d\big)+\log\big(\frac{1}{\epsilon}\big) \Big)}&\text{ when } r<\sqrt{d/2}\\
\BO{n\Big(r\log\big(d\big)+\log\big(\frac{1}{\epsilon}\big) \Big)}&\text{ when } \sqrt{d/2}\leq r \leq d/3\label{eq:4}
\end{align}
and $|\cup_{x\in S}B(x,cr)|<2^{d-1}$.
\begin{proof}


Recall definition \ref{def:EDSAM}. Given a set $S$ of size $n$, a valid filter could be constructed by storing at most $n$ balls, $A_1,..,A_n$, selected so that:
\begin{enumerate}  
\item   For each $x\in S$ there is some $A_i$ such that $x\in A_i$.
\item   And the distance from $x$ to the edge of $A_i$ is at least $r$. \alertF{is edge of a ball defined?}
\item   $|\cup A_1,..,A_n|\leq \big(2^d-\cup_{x\in S}B(x,cr)\big)\epsilon+\cup_{x\in S}B(x,cr)$ 
\end{enumerate}
  
A query $q$ would be answered positively if there is some $A_i$ such that $q\in A_i$ and otherwise negatively.
We see that the first two requirements guarantee there will no false negatives, and the third that there won't be too many false positives.

We want to choose the largest $A_i$ balls possible without breaking the third requirement.
Assuming all $A_i$ have the same volume it would be:
\[
  |A_i|=(2^d-\cup_{x\in S}B(x,cr))\frac{\epsilon}{n}+B(cr)\geq 2^{d-1}\frac{\epsilon}{n},    
\]
if we assume that the total space covered by $\cup_{x\in S}B(x,cr)$ is less than $2^{d-1}$.


We will represent each ball $A_i=B(q_a,r_a)$ by a smaller ball $A_i^{-r}=B(q_a,r_a-r)$, so that if $x\in A_i^{-r}$ it fulfills both requirements.

The rest of the proof will progress as follows: First we will determine how large $A_i^{-r}$ can be, and we will then bound the size of a covering of the space by such balls.
An upper bound on storage is then given by the size of representing a specific choice of $n$ balls from the covering.

To find the radius of $A_i$ we want to select an $\epsilon/n$ fraction of the $d'=d-1$ dimensional hamming cube in a ball.
We can use the basic fact about the relationship bewteen the hamming ball and the Binonimal distribuition:

  \begin{lemma}[Hamming ball volume]
    \label{lem:BallVolume}
    By the definition of the radius $r\geq 0$ ball in $d$ dimensional hamming space: \alertF{The proof shouldn't be inside a lemma/theorem statement, even if trivial.}

    \[|B(r)|=\sum_{i=0}^{r}{d \choose i}=2^d\Pr[X\leq r] \text{ for } X\sim B(d,1/2)\]
where $B(d,p)$ is the binomial distribution.
\end{lemma}
    
This is usefull since we have thight bounds for the binomial distribution.
Particularly:
\begin{lemma}[Chernoff Bound]
  \label{lem:Chernoff}
  Let $X\sim B(d,1/2)$:

  \[
    \Pr[X\leq \frac{d}{2}-a]\leq e^{-2a^2/d}\text{ for } 0\leq a \leq d/2
    \]
\end{lemma}

So it's safe to set the radius of $A$ to at least $d/2-a$ where $a=\sqrt{\frac{d'\log(n/\epsilon)}{2}}$ since:
\[
  |B\big(\frac{d'}{2} - a\big)|=2^{d'}\Pr\Bigg[X\leq \mu - \sqrt{\frac{d'\log(n/\epsilon)}{2}}\Bigg]\leq 2^{d'}\epsilon/n
\]
Where $\mu = \E[X] = \frac{d'}{2}$.
We can express the radius of $A$ in terms of the number, $\lambda_a=\sqrt{2\log(n/\epsilon)}$, of standard deviations $X$ is from $\mu$.
Recall that the standard deviation for $B(d',0.5)$ is $\sqrt{d'}/2$, so the radius of $A^{-r}$ is at least:

\[
  \mu-(\lambda_a)\frac{\sqrt{d'}}{2}-r
\]

If we represent $r$ as a number of standard deviations,$\lambda_r=2r/\sqrt{d'}$, we find that the radius of $A^{-r}$ is at least:

\[
  \mu-(\lambda_a+\lambda_r)\frac{\sqrt{d'}}{2}
\]

Here's Berry-Essen:
  \begin{lemma}[Berry-Esseen]
    \label{lem:BerryEsseen}
    Let $X\sim B(d,1/2)$ and $x\in \BO{1}$:
\[
    \Phi(-x)-\frac{C}{\sqrt{d}}\leq\Pr[X\leq \frac{d}{2}-x\frac{\sqrt{d}}{2}]\leq \Phi(-x)+\frac{C}{\sqrt{d}}
  \]

  Where $\Phi(x)$ is the CDF of $\mathcal{N}(d/2,\sqrt{d}/2)$.
  $0.409732..\leq C \leq 0.4215$ by \cite{Nagaev2011}.
\end{lemma}
 
Now by lemma \ref{lem:BerryEsseen}:


\alertF{You should be sure that $C/\sqrt{d}$ is really negligible and not larger than $\Phi(x)$ for very small values of $x$ (I had this problem in my proof). Note that I use Berry-Esseen in the signature: if this section remains in the paper, we should not introduce Berry-Essen twice. 
Also I think it is not needed to use in a conference paper  full lemmas to introduce Chernoff bounds and Berry Esseen since they are well known (at least Chernoff bounds!).
}

\alertF{There is a big discontinuity here since the proof moved from a combinatorial approach to a probabilistic one. You should add more explanations.}

\begin{align}
  \Pr[X\leq\mu-(\lambda_a+\lambda_r)\sqrt{'d}/2]\approx  \frac{1}{\sqrt{2\pi}}\int_{-\infty}^{-\lambda_a-\lambda_r}e^{-t^2/2}dt=\\
    \frac{1}{\sqrt{2\pi}}\int_{-\infty}^{-\lambda_a}e^{-t^2/2}dt-\frac{1}{\sqrt{2\pi}}\int_{\lambda_a-\lambda_r}^{\lambda_a}e^{-t^2/2}dt)
\end{align}

Again by \ref{lem:BerryEsseen} and \ref{lem:Chernoff}:
\[
  \frac{1}{\sqrt{2\pi}}\int_{-\infty}^{-\lambda_a}e^{-t^2/2}dt\approx\Pr[X\leq \mu-\lambda_a\frac{d'}{2}]\leq\epsilon/n
\]

So by inserting:
\[
  \Pr[X\leq\mu-(\lambda_a+\lambda_r)\sqrt{d'}/2]\approx \epsilon/n - \frac{1}{\sqrt{2\pi}}\int_{-\sqrt{2\log(n/\epsilon)}-\lambda_r}^{-\sqrt{2\log(n/\epsilon)}}e^{-t^2/2}dt
\]

Simplifying and inserting $\lambda_r=2r/\sqrt{d'}$ we get:

\[
 \frac{|A_i^{-r}|}{2^{d'}}\approx \epsilon/n-1/2\Big(\text{Erf}(\frac{\sqrt{2}r}{\sqrt{d'}}+\sqrt{n/\epsilon})-\text{Erf}(\sqrt{n/\epsilon})\Big)
\]


Lets first look the the case where the volume is dominated by $\epsilon/n$, looking at the error function this happens if $\sqrt{n/\epsilon}$ is larger than $\approx 2$\jnote{This seems like a too relaxed bound. eps should be smaller than that i think}, no matter how large $r$ is, or if $\sqrt{n/\epsilon}$ is around $1$ or smaller i.e. $\epsilon\approx 1/n$ if $r<<\sqrt{\frac{d'}{2}}$.
So for $r<\sqrt{\frac{d-1}{2}}$ we will use $|A_i^{-r}|\in\BOM{2^{d-1}\epsilon /n}$

If the loss of volume from $r$ is substantial we can give another bound on the volume of $A_i^{-r}$:
\begin{lemma}
\label{lem:sphere in spheres}
Given a hamming ball $A=B_d(C_a,r_a)$ and a point $x\in A$. Let $d\geq r$.
\begin{equation}
\forall r<r_a\exists \lambda \text{ such that } B_d(\lambda,r)\subseteq A \text{ and } x\in B_d(\lambda,r)
\end{equation}
\begin{proof}
Take $XOR(x,C_a)$ and for the $r$ first non-zero entries flip the corresponding entry in $x$. Call the resulting vector $\lambda$. If $|XOR(x,C_a)|<r$ let $\lambda = C_a$.
Now $D(x,\lambda )\leq r$ so $x\in B(\lambda ,r)$. 
At the same time $D(C_a,\lambda )\leq r_a-r$ so the distance between $C_a$ and any point on $B(\lambda, r)$ is at most $r_a$.
Therefor $B(\lambda,r)\subseteq A$.
\end{proof}  
\end{lemma}

\begin{lemma}
\label{lem:sphere_contains}
A $d$ dimensional hamming sphere $A$ of radius $r_a$ can fully contain at least 
\begin{equation}
\frac{|A|}{\sum_{i=0}^r{d \choose i}}
\end{equation}
spheres of radius $r\leq r_a$.

\begin{proof}
Let $\lambda$ denote the set of center points of radius $r$ spheres fully contained in $A$. 
Since every point in $A$ lies within radius $r$ of some point in $\lambda$ (by lem.~\ref{lem:sphere in spheres}) we have $|\lambda|\sum_{i=0}^{r}{d \choose i}\geq |A|$.
\end{proof}
\end{lemma}

So for $r\geq \sqrt{\frac{d-1}{2}}$ we can use $|A_i^{-r}|$ is $\BOM{\frac{2^{d'}}{\sum_{j=0}^r{d \choose j}}}$.

To upper bound the size of the datastructure we will first determine how large a covering of the entire hamming space $\{0,1\}^d$ will be in these two settings of $A_i^{-r}$.

\begin{lemma}
\label{lem:random_covering}
There exists a covering of the $\{0,1\}^d$ space using $d2^d/V$ sets of volume $V$.
\begin{proof}
If we place $t$ sets at random the probability that a random point from $\{0,1\}^d$ is not covered is 
\begin{equation*}
(1-\frac{V}{2^d})^t\leq e^{-\frac{V}{2^d}t}
\end{equation*}
So by the union bound the probability that any point is left uncovered is bounded by
\begin{equation*}
2^de^{-\frac{V}{2^d}t}\leq 0.8
\end{equation*}
If we set $t=d\frac{2^d}{V}$.
\end{proof}
\end{lemma}

If we want a valid datastructure for all possible inputs, by lemma \ref{lem:random_covering} theres is some covering, $C$, of the space possible where the number of such balls is:
\begin{align}
   |C|&=d\frac{2^d}{|A_i^{-r}|}\rightarrow\\
      |C|&\leq\frac{dn}{\epsilon}\text{ for } r<\sqrt{(d-1)/2}\\
  |C|&\leq\frac{d2(ed/r)^rn}{\epsilon}\text{ for } \sqrt{(d-1)/2}<r<d/3 
\end{align}

 When processing an input set $S$ of size $n$ we would need to find and store the indexes associated with at most $n$ balls containing a full $B(x,r)$ associated with each $x\in S$. 
So a valid data structure is simply to distinguish which size $n$ subset corresponds to $S$ , requiring space:

\[
  \BO{\log{{|C|\choose n}}}=
\begin{cases}
  \BO{n\Big(\log\big(d\big)+\log\big(1/(\epsilon\big) \Big)}\text{ for } r<\sqrt{(d-1)/2}\\
  \BO{n\Big((r+1)\log\big(d\big)+\log\big(1/(\epsilon\big) \Big)}\text{ for } \sqrt{(d-1)/2}<r<d/3
\end{cases} 
\]

Note that we rely on a non-constructive existence proof for the cover, however for a given $d$ a more efficient cover will often be available.
\end{proof}
\end{theorem}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> definition.tex <==
 \section{Locality Sensitive Approximate Membership}
\subsection{Worst case error version (LSAM)}
For $r>0$, $\epsilon\in[0,1]$,$c\geq 1$. 
Given a set $S\subseteq X$,  a datastructure solves the $(c,r,\epsilon)$-LSAM problem if when queried with some $q\in X$ it reports: 

\begin{itemize}
\item \emph{Yes} if $D(q,S)\leq r$. 
\item  \emph{No} with probability at least $1-\epsilon$  if $D(q,S)\geq cr$.
\end{itemize}

If $r<D(q,S)<cr$ the datatstructure may give any answer.

The problem is defined for any metric space $(X,D)$, in this paper we will focus on addressing it in $(\{0,1\}^d,\mathbb{H})$.

\subsection{Expected error version (ELSAM)}

Since the purpose of the datastructure is to discriminate points based on their proximity to points in $S$ it seems natural to allow the error probability to depend on this. 
We allow the structure to fail more often on near than far points and only promise bounds on the expected error:\\
For  $r>0$, $\epsilon \in [0,1]$. 
Given a set $S\subseteq X$ a datastructure solves the $(r,\epsilon)$-ELSAM  problem if  when queried with some $q\in X$ it reports: 

\begin{itemize}
\item \emph{Yes} if $D(q,S)\leq r$. 
\item  \emph{No} with expected probability at least $1-\epsilon$  if $D(q,S)> r$.
\end{itemize}

Where the expectation is over $q\in X\setminus\{\cup_{x\in S} B(x,r)\} $. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> makefile <==
SHELL = bash
SRC = $(wildcard illustrations/*.mp)
SUBSRC = $(patsubst illustrations/%.mp,%.mp,$(SRC))

mp :
	cd illustrations;for file in $(SUBSRC) ; do \
		mpost -tex=latex $$file ; \
	done

pdf : mp $(SRC)
	pdflatex main.tex
	pdflatex main.tex
	okular main.pdf

clean :
	$(RM) main.pdf *.log *.aux *.out *.bbl *.blg *.toc *.nav main.snm
	mv illustrations/*.mp .
	$(RM) illustrations/*
	mv *.mp illustrations/



==> notation.tex <==
\subsection{Notation}
\begin{itemize}
\item In a $(X,D)$ metric space, given a set $S\subseteq X$ and a point $q\in X$ let $D(q,S)$ = $\min_{x\in S}D(q,x)$.
\item Let $B_d(r)$ denote a radius $r$ hamming ball in $d$ dimensions, and $B_d(x,r)$ be a radius $r$ ball centered in $x$.
\item Let $S_d(r)$ denote the surface area of $B_d(r)$.
\item $\mathbb{H}$ is the Hamming distance.
\end{itemize}


==> overview.tex <==
\subsection{Average case}

In the average case we guarantee that at most an $\epsilon$ fraction of the points $\notin \{\cup_{x\in S}B(x,r)\}$ are accepted. 
$$
\BO{n\Big(r\log\big(d\big)-\log\big(\frac{\epsilon}{n}+\frac{(1-\epsilon){d \choose r}}{2^{d}}\big) \Big)}$$
 when $r\leq d/2-\sqrt{d}$.

$$\Omega \Big( n\big(r \log(d) - \log (\epsilon+ \frac{n {d \choose r}}{2^{d-1}}) \big)\Big)$$
where $r<d/3$.

\subsection{Worst case}

In the worst case we guarantee that any point $\notin \{\cup_{x\in S}B(x,cr)\}$ is accepted w.p $\leq \epsilon$.

\subsubsection{Lower bound}
Based on the promised existence of error correctiong codes with the properties:

\begin{itemize}
\item $1/(r\epsilon)^2$ code words
\item Each of length $d/k$
\item And weight $r/k$
\item Minimum distance betwenn codewords $r(c-1)$
\end{itemize}

Two codewords compared by table 1:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> prior.tex <==
\subsection{Prior work}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

There is some prior work in membership structures that incorporate locality \cite{Kirsch}, \cite{Hua2012}.
Efforts here have been focused on constructing Bloom filters\cite{Qiao2014},\cite{Carter1978} but using locality sensitive hash functions\cite{Gionis1999} to make the filters distance sensitive. 

However one of the main benefits of Bloom filters is the lack of false negatives. 
Having only false positives makes Bloom filters useful in many practical scenarios where a few false positives are acceptable, but avoiding false negatives crucial.
Unfortunately the hash functions used in both \cite{Kirsch} and \cite{Hua2012} introduce false negatives.

